Robust Multi-Modal Multi-LiDAR-Inertial Odometry and Mapping for Indoor Environments

Integrating multiple LiDAR sensors can significantly enhance a robot's perception of the environment, enabling it to capture adequate measurements for simultaneous localization and mapping (SLAM). Indeed, solid-state LiDARs can bring in high resolution at a low cost to traditional spinning LiDARs in robotic applications. However, their reduced field of view (FoV) limits performance, particularly indoors. In this paper, we propose a tightly-coupled multi-modal multi-LiDAR-inertial SLAM system for surveying and mapping tasks. By taking advantage of both solid-state and spinnings LiDARs, and built-in inertial measurement units (IMU), we achieve both robust and low-drift ego-estimation as well as high-resolution maps in diverse challenging indoor environments (e.g., small, featureless rooms). First, we use spatial-temporal calibration modules to align the timestamp and calibrate extrinsic parameters between sensors. Then, we extract two groups of feature points including edge and plane points, from LiDAR data. Next, with pre-integrated IMU data, an undistortion module is applied to the LiDAR point cloud data. Finally, the undistorted point clouds are merged into one point cloud and processed with a sliding window based optimization module. From extensive experiment results, our method shows competitive performance with state-of-the-art spinning-LiDAR-only or solid-state-LiDAR-only SLAM systems in diverse environments. More results, code, and dataset can be found at \href{https://github.com/TIERS/multi-modal-loam}{https://github.com/TIERS/multi-modal-loam}.

==> sec/00_AB_OLD.tex <==

\begin{abstract} 
% The integration of multiple LiDAR sensors allows a robot to significantly enhance its perceptual awareness of the environment and capture sufficient measurements, making it a promising approach for simultaneous localization and mapping (SLAM).
Integrating multiple lidar sensors can significantly enhance a robot's perception of the environment, enabling it to capture adequate measurements for simultaneous localization and mapping (SLAM).
% 
% Solid-state LiDAR is gaining more attention due to its high resolution and low cost, making it a viable option for various robotic applications across different environments. However, its limited field of view (FOV) can hinder performance in indoor environments where nearby objects can occlude part of the FOV, leading to ego-motion estimation failure, furthermore novel non-repetitive scanning pattern provide dense measurements points which able to scan same objects within FOV and require novel methods to accurately un-distort the points and align the points for same object.
% In contrast, traditional spinning LiDAR offers a 360-degree horizontal FOV, but its low vertical resolution can lead to matching errors along the Z-axis.
% 
% Solid-state lidar's high resolution and lower cost offer advantages over traditional spinning LiDAR for robotic applications, but its limited field of view (FoV) may hinder performance in indoor environments. 
 Indeed, solid-state lidars can bring in high-resolution at low cost to traditional spinning lidars in robotic application. However, their reduced field of view (FoV) limits performance, particularly indoors.
% Furthermore, Novel scanning patterns generate dense point cloud data, but require innovative un-distortion methods. Traditional spinning LiDAR usually has a larger horizontal FOV, but limited vertical resolution can cause errors along the Z-axis.
% 
In this paper, we propose a tightly-coupled multi-modal multi-lidar-inertial SLAM system for surveying and mapping tasks. By taking advantage of both solid-state LiDARs, spinning s, and built-in inertial measurement units (IMU), we achieve both robust and low-drift ego-estimation as well as high-resolution maps in diverse challenging indoor environments (e.g., small, featureless rooms).
% 
% The proposed system can be divided into for-end and back-end. For the foreend
First, we use spatial-temporal calibration modules to align the timestamp and calibrate extrinsic parameters between sensors.
Then, we extract two groups of feature points including edge and plane points, from LiDAR data.
% Then, a plane feature based un-distortion module is employed on solid-state LiDAR pointcloud data. [Might be in the future]
Next, with pre-integrated IMU data, an undistortion module is applied to the LiDAR pointcloud data. 
Finally, the undistorted pointclouds are merged into one point cloud and processed with a sliding window based optimization module.
% together with the plane feature map from backend and IMU data, the ego-motion are estimated for both spinning LiDAR and solid-state LiDAR. 
% The extracted features are scored based on the feature's spatial distribution, amount, and rotation constraints, and the higher-scored feature cloud will be utilized in the mapping process.
% In the back-end, sliding window optimization and graph optimization are used to achieve global consistent mapping.
% A graph is also built based on a sub-map, loop closure optimization is conducted when a close loop is detected. 
% 
% We evaluate the proposed method in our datasets logged by the backpack across different scales and environments. Furthermore, the TIERS LiDARs dataset is used to benchmark our method quantitatively. 
From extensive experiment results, our method shows competitive performance with state-of-the-art spinning-LiDAR-only or solid-state-LiDAR-only SLAM systems in diverse environments. More results, code, and dataset can be found at \href{https://github.com/TIERS/multi-modal-loam}{https://github.com/TIERS/multi-modal-loam}.

\end{abstract}

\begin{IEEEkeywords}
    LiDAR-inertial odometry, multi-LiDAR systems, sensor fusion, solid-state LiDAR, SLAM, mapping
 
\end{IEEEkeywords}

==> sec/01_INT_OLD.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                                          %%
%%              INTRODUCTION                %%
%%                                          %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
% 02/28- 3/1: Recheck, Review and Update

\section{Introduction}
\label{sec:introduction}

Autonomous mobile robots rely heavily on spinning 3D LiDAR sensors, which offer high-quality geometric data at long ranges, with a full horizontal FoV, and robust performance across environmental conditions. As a result, this technology has found widespread application in a variety of fields, including self-driving vehicles~\cite{li2020multi}, unmanned aerial vehicles~\cite{varney2020dales}, and forest surveying systems~\cite{yang2020individual, li2020localization}, among other areas.

\begin{figure}[t]
    \centering 
    \begin{subfigure}{0.45\textwidth}
        \centering 
        \includegraphics[width=\textwidth]{fig/first-figure.png} 
        \caption{Mapping result with the proposed system at a hall environment. Thanks to the high resolution of solid-state LiDAR with a non-repetitive scan pattern, the mapping result is able to show clear detail of object's surface.}  
        \label{fig:hall_mapping} 
    \end{subfigure}
    
    \vspace{0.5em}
    
    \begin{subfigure}{0.45\textwidth}
        \centering 
        \includegraphics[width=\textwidth]{fig_iros/second-figure4.png} 
        \caption{Hardware and Mapping result in long corridor environment. Our proposed methods show robust performance in long corridor environment and survive in narrow space where 180\degree U-turn occurs.}  
        \label{fig:corridor_mapping} 
    \end{subfigure}
    
    \caption{Our proposed methods show high-resolution mapping results and robust performance in challenging environment}
\end{figure}

In odometry and mapping tasks, achieving denser 3D geometry measurements of the surrounding environment is crucial for enhancing 3D environment understanding. Unfortunately, spinning LiDAR with higher resolution and multiple beams can be costly due to its more complicated architecture. Low-resolution spinning LiDAR, while more affordable, produces sparse point clouds with limited features, making the problem difficult to tackle~\cite{ye2019liomap} and leading to inevitable inherent alignment errors~\cite{xu2022robust}.
  
LiDAR technology has advanced rapidly in recent years, with new sensors able of generating image-like data in additon to pointclouds~\cite{tampuu2022lidar, xianjia2022analyzing}, and new solid-state LiDAR sensors that offer dense 3D pointclouds with non-repetitive scan patterns, while at the same time lowering the cost~\cite{lin2020loam, li2021towards}. 
% In recent times, solid-state LiDAR has generated significant interest due to its high resolution and cost-effectiveness~\cite{lin2020loam, li2021towards}. Unlike conventional low-resolution spinning LiDARs, it employs an incomparable scanning pattern that enables it to produce much denser resolution~\cite{liu2021lowretina}.
% On the other side, its unique features also challenge the traditional LiDAR-based localization and mapping methods with a small FoV, irregular scanning pattern, non-repetitive scanning and motion blur.
Despite the clear advantages of solid-state LiDARs, 
%including its high resolution and cost-effectiveness, 
the naturally narrow horizontal FoV leads, in a similar way to monocular pinhole camera systems, to the sensing volume being blocked by objects, or even entirely occupied by a near wall, resulting in an insufficient number of feature points to estimate a 6-DoF pose. This limitation has made current solid-state-based SLAM methods challenging to apply in outdoor or large indoor scenarios~\cite{li2021towards, sier2022benchmark}. 

% multi lidars fusion
% To enhance the robustness of autonomous systems, researchers have tried to 
Multiple works in the literature have been directed towards improving LiDAR maps by merging point clouds from multiple LiDAR sensors. However, this process requires precise time synchronization and extrinsic calibration to align the two points accurately in both temporal and spatial spaces~\cite{chen2021backpack}. When hardware time synchronization is unavailable, the low publishing frequency of LiDAR frames (e.g., 10\,Hz) can impede the estimation of time offset between the LiDARs. There is a lack of methods that are able to leverage multi-LiDAR systems for odometry estimations.
% To address this issue, we propose a method that maintains the two original data formats throughout the process and jointly optimizes the pose during the optimization steps. [Methods changed]
 


% \begin{figure}[t]
%     \centering 
%     \includegraphics[width=0.5\textwidth]{fig/mapping_result_com.jpg} 
%     \caption{Mapping result comparison on sequence Indoor00. (Top-left map) Lego-LOAM with low resolution spinning lidar; (Bottom-left) LIO-LIVOX by solide-state lidar with in non-repetition scanning pattern;(Right) our proposed tightly coupled multi-modal lidar inertial odometry and mapping method. By taking advantage of the large horizontal FoV from spinning lidar, high resolution in vertical FoV from solid-state-lidar and an low-cost built-in IMU, our proposed method achieved state-of-the-art performance \red{TODO}} 
    
%     \label{fig:mapping_comprision} 
% \end{figure}

% % Calibraition
%  Different sensors can complement each other and the overall perception capability will be significantly improved with sensor fusion. For example, inertial measurement units (IMUs) feature a high update rate but noisy and drifting sensor data, cameras have high-resolution passive perception but suffer from image blur and scale ambiguity, while Lidars have accurate depth perception ability but limited horizontal resolution and field of view (FoV). To realize valid and robust sensor fusion, sensor data synchronization of different sensors are crucial to such a fusion-based system. In order to achieve high-precision synchronization and calibration, we leverage the high update rate of the IMU and design an IMU-centric calibration scheme, as shown in Fig. 1. 

%  The feature quality and its impact on mapping result has not been discussed thoroughly. Especially, the novel solid state lidar with non-repetition patterns bring high resolution in its FoV with low-cost. However, their accurate mapping ability hasn't been fully explored, especially in cluttered environment,  which require new methods to adapt new feature.

%  Our method
To improve the robustness of the SLAM system, we propose a novel tightly-coupled multi-modal multi-LiDAR-inertial odometry and mapping system, which takes advantage of both the large horizontal FoV from a spinning LiDAR and the dense measurements from a solid-state LiDAR. 
% The proposed system can be divided into for-end and back-end. For the foreend,
% First, a union feature extraction method are used to extract feature points(edge, corner, and plane) from lidar data.
% Then, a plane feature based un-distortion module is employed on solid-state Lidar pointcloud data. Next, together with the plane feature map from backend and IMU data, the ego-motion are estimated for both spinning lidar and solid-state lidar. 
% % The extracted features are scored based on the feature's spatial distribution, amount, and rotation constraints, and the higher-scored feature cloud will be utilized in the mapping process.
% In the back-end, sliding window optimization and graph optimization are used to achieve global consistent mapping. 
The proposed system first performs spatial-temporal calibration to calibrate the time-offset and extrinsic parameters between sensors.
Then, we extract two group feature points, continuous and discontinuous points, or edges and planes, from lidar data.
% Then, a plane feature based un-distortion module is employed on solid-state Lidar pointcloud data. [Might be in the future]
Next, with pre-integrated IMU data plane feature based un-distortion module is employed on Lidar pointcloud data. 
Finally, the un-distorted pointcloud are merged into one point cloud and sent to sliding window based optimization module 

%  \blue{Most of the previous work considers
% the distortion arising from successive frames (inter-frame)
% while ignoring the distortions occurred within each frame
% (intra-frame), as they are relatively small for the 360° rotating
% lidars. Assuming a moving object has 20° angular extension
% and lidar operates at 10 Hz (100 ms frame duration), the
% total scan time of the object in one frame is roughly
% 100 ms × (20°/360°) = 5.6 ms. On the other hand, the
% oscillating lidars could have points describing that object
% coming from anywhere of the 100 ms frame duration (Fig. 1).
% As a result, the previous methods did not accommodate these
% severe intra-frame distortions from the oscillating type lidars.}

This work is, to the best of our knowledge, the first lidar-inertial SLAM system to effectively integrate lidar sensors with heterogeneous scan modalities within a single estimation and optimization framework. This work is inspired by the limitations found in state-of-the-art algorithms for different lidar sensors in our previous works~\cite{li2022dataset,sier2022benchmark}, where low-cost solid-state lidar outperform high-resolution spinning lidar in an outdoor environment, but at the same time perform poorly in indoor environments. 
% In this paper, we introduce \red{feature extraction failure detection, multi-modal lidar online calibration} method, to tackle two key issues that degenerate the SLAM system. 
 % 
The unique characteristics and main contributions of our work can be summarized as follows: 
\begin{enumerate} 

    % \item We proposed a low-drift real-time SLAM framework for handhold device by fusion spinning lidar and solid-state-lidar and has been validated by extensive experiments. \red{Robustness and Extendibility}

    % \item High-resolution and sharp pointcloud map assisted by novel un-distortion methods for multi-modal multi-lidar systems.
    
    \item Design and implementation of a novel tightly-coupled multi-modal multi-lidar-inertial mapping framework that is able to combine lidars with different scanning modalities for odometry estimations.
    
    \item The demonstration of a SLAM method for taking advantage of low-cost spinning lidars and solid-state lidars that outperform the state-of-the-art in high-resolution mapping with high levels of detail.

 
    % \item A data-driven deep learning based semantic environment localization and mapping methods are introduced by leveraging the advantages of dense pointcloud measurement from solid-state-lidar and large FoV from spinning lidar
    % \item We presented group truth map generation methods with non-repetitive scanning pattern by solid-state-lidar.
    
    % \item Adaptive voxel map resolution with intensity information aided object level map are introduced, which contain the motion probability of each object, which can indicate the map quality and potential change of map. The optimized ground info can provide abundant infomartion for different platform, specially for quadpedal robot. 
    
    % \item This is the first open-source implementation for tightly coupled multi-modal lidar and IMU fusion available to the community. Through extensive experiments, our proposed methods show state-of-the-art ability in a diverse environment.
    
    %  % \item range image projection methods
    % \item Degenerate Motion Analysis, in this paper, we discussed the degenerate motion environment, and how our proposed fusion method can improve system performance

    % \item \blue{ We proposed a unified feature extraction algorithms which can be shared by diverse lidar. With carefully selected feature points, the total number of feature points is also reduced.}
    
\end{enumerate}

We provide a unique open-source implementation for tightly-coupled multi-modal lidar and IMU fusion available to the community. Through extensive experiments, our proposed methods show state-of-the-art capabilities in various environments, with comparable odometry estimations and higher map quality. The structure of the paper is as follows. Section II surveys the existing research in multi-lidar systems and mapping and SLAM with solid-state lidar. Section III introduces our proposed mythology. Section IV delves into the details of the implementation and experimental results. Finally, Section V concludes the study and suggests future work.

 

==> sec/02_REL_OLD.tex <==
 

\begin{table}[t]
    \centering
    \caption{Characterization of off-the-shelf lidar sensors based on horizontal resolution (H. Res.), vertical resolution (V. Res.) and cost.}
    %H. Reso.: Horizontal resolution; V. Reso.: Vertical resolution; HR. : High resolution; LR.: Low resolution } 
    \begin{tabular}{@{}lccc@{}}  
    \toprule 
        Lidar Types       & \textbf{High H. Res.}     & \textbf{High V. Res.}  & \textbf{Low-cost}           \\[0.5ex]
     \midrule     
        Spinning, 64+ channels    & \CheckmarkBold    & \CheckmarkBold    & \XSolidBrush      \\[0.5ex]
        Spinning, 16-32 channels    & \CheckmarkBold    & \XSolidBrush      & \CheckmarkBold    \\[0.5ex] 
        Solid-State     & \XSolidBrush      & \CheckmarkBold    & \CheckmarkBold    \\[0.5ex]  
    \bottomrule 
    \hspace{.42em}
    \end{tabular}    
    \label{table:lidars_comp}
\end{table} 
 

\section{Related Works}
\label{sec:related_works} 

% \red{1. Feature based lidar odometry and mapping; 2. Solid-lidar based SLAM; 3. Multi-lidar SLAM}

\subsection{Feature-based LiDAR odometry and mapping}

LiDAR odometry generally employs scan-matching techniques including ICP, KISS-ICP~\cite{vizzo2023kiss}, GICP~\cite{segal2009gicp}, and others to determine the relative transformation between two successive frames.
% Lidar odometry is typically performed by finding the relative transformation between two consecutive frames using scan-matching methods such as ICP, KISS-ICP~\cite{vizzo2023kiss}, and GICP~\cite{segal2009gicp}.
Feature-based matching approaches have gained popularity as a computationally efficient alternative to full point cloud matching.
% Instead of matching a full point cloud, feature-based matching methods have become a popular alternative due to their computational efficiency
For example, in~\cite{zhang2014loam}, Zhang et al. propose the registration of edge and plane features for real-time LiDAR odometry. This type of operation assumes that the LiDAR moves within a structured environment, with edge and plane points clearly identifiable from the point clouds. The matching of consecutive scans is then performed by solving a least-squares optimization problem.  
SLAM with features of planes for indoor environments has attracted many researchers' interests as planes ubiquitously exist in indoor environments~\cite{zhou2021plane}. 


\subsection{SLAM with solid-state LiDARs}\label{sec:solid_state}  

With the development of LiDAR technology, low-cost and high-performance solid-state LiDAR has attracted significant researcher interest. The different sensing characteristics means that new challenges in pointcloud registration and mapping arise. In~\cite{lin2020loam}, Lin et al. address several fundamental challenges with a robust, real-time LiDAR odometry and mapping algorithm for solid-state LiDAR (LOAM Livox) that accounts for the reduced FoV and the non-repetitive sampling patterns has been presented by taking effort on both front-end and back-end in. Other recent results have also presented tightly-coupled LiDAR-inertial odometry and mapping schemes for both solid-state and mechanical LiDARs~\cite{li2021towards, xu2021fast}. Regarding the inherently limited FoV  of a single solid-state LiDAR, a decentralized approach for simultaneous calibration, localization, and mapping utilizing multiple solid-state LiDARs was introduced in~\cite{lin2020decentralized} to enhance system resilience.

% A decentralized framework for simultaneous calibration, localization, and mapping with multiple solid-state LiDARs has been proposed in~\cite{lin2020decentralized} to solve the small FoV problem of single solid-state LiDARs and improve the system robustness.   
% c
% 
% 
% In~\cite{liu2021balm},  inspired by a local Bundle Adjustment (BA) on a sliding window of keyframes which has been widely used in visual SLAM, the author proposed a BA method with an adaptive voxelization method to search feature correspondence to solve the sparse features points of LiDAR data.
% 
% 

\begin{figure}[t]
    \centering  
     \includegraphics[width=0.48\textwidth]{fig_iros/flow-chart3.png}
    \caption{ The pipeline of proposed multi-modal lidar inertial odometry and mapping framework.
    The system starts with preprocessing module where takes the input from sensors and performs IMU pre-integration, calibrations and un-distortions. 
    The scan registration module extracts features and sent the features to a tightly coupled sliding window odometry. Finally, a pose graph is built to maintain global consistency. } 
    \label{fig:sys_overview} 
\end{figure} 

\begin{figure}[t]
    \centering  
    \includegraphics[width=0.48\textwidth]{fig_iros/feature_pts1.png}
    \caption{Extracted features points in office room environment(left) and zoom-in view of one gate object (right). plane and edge feature points from Velodyne are in red and blue, plane and edge feature points from Horizon are in green and white separately}
    \label{fig:feature_pts} 
\end{figure} 


\begin{figure}[t]
    \centering  
    \includegraphics[width=0.45\textwidth]{fig_iros/extrinsic_cali2.png}
    \caption{Lidars extrinsic parameter calibration result in an office room environment. Red point cloud come from Horizon and green point cloud from VLP-16.(left) top view (right) detail of the matching }
    \label{fig:extrin_cali} 
\end{figure}

\subsection{Multi-modal LiDAR-based SLAM}

Relying solely on spinning LiDARs for pose estimation is suboptimal, as registering skewed point clouds or features can eventually result in substantial drift. Contemporary LiDAR SLAM systems commonly integrate data from multiple sensors to enhance accuracy. LIO-SAM was proposed as a method to eliminate the accumulated drift of LiDAR-inertial odometry over extended periods or in feature-sparse environments, by tightly coupling LiDAR and inertial measurement unit (IMU), and optionally GNSS sensors, via smoothing and mapping~\cite{shan2020lio}. SLAM approaches utilizing the fusion of LiDAR and IMU data can be found in other studies, for example, LIO-Mapping~\cite{ye2019tightly} and Fast-LIO with iterated Kalman filter~\cite{xu2021fast}. Moreover, integrating LiDAR-inertia odometry with visual-inertia odometry (VIO) can further improve accuracy while keeping the robustness either in  texture-less or feature-less environments~\cite{shan2021lvi}.


% Tightly-coupled systems usually offer improved accuracy
% and are presently a major focus of ongoing research [14].
% In [15], preintegrated IMU measurements are exploited for
% de-skewing point clouds. A robocentric lidar-inertial state
% estimator, R-LINS, is presented in ~\cite{qin2020lins}. R-LINS uses an
% error-state Kalman filter to correct a robot’s state estimate
% recursively in a tightly-coupled manner. Due to the lack
% of other available sensors for state estimation, it suffers
% from drift during long-during navigation. A tightly-coupled
% lidar inertial odometry and mapping framework, LIOM, is
% introduced in ~\cite{ye2019liomap}. LIOM, which is the abbreviation for
% LIO-mapping, jointly optimizes measurements from lidar and
% IMU and achieves similar or better accuracy when compared
% with LOAM. Since LIOM is designed to process all the
% sensor measurements, real-time performance is not achieved
% - it runs at about 0.6× real-time in our tests.


\subsection{Multi-LiDAR odometry and mapping}

More recently, research focus has also shifted towards the fusion of data from multiple lidars. For example, \cite{jiao2021robust}~addresses multi-LiDAR online extrinsic calibration, odometry, and mapping, where extracted edge and planar features are utilized  and data uncertainty is modeled with Gaussian distribution. A tightly coupled LiDAR-inertial odometry and mapping approach with low drift is proposed in~\cite{nguyen2021miliom}, which utilizes features extracted from multiple time-synchronized LiDARs with complementary FoV. Rather than utilizing spinning LiDARs, a decentralized extended Kalman filter (EKF) approach for simultaneous calibration, localization, and mapping for multiple solid-state LiDARs was introduced to improve upon the limited FoV of a single solid-state LiDAR~\cite{lin2020decentralized}. However, we find a lack of work in the literature in terms of fusing multiple lidars with different scanning modalities, which has potential due to the different advantages they have in terms of map quality and odometry accuracy.

%the technique of fusing multiple LiDARs with differing modalities for odometry and mapping has not been widely utilized thus far.
% There are multiple work on fusing LiDARs with different modalities.
% Robust Odometry and Mapping for Multi-LiDAR Systems With Online Extrinsic Calibration are proposed in~\cite{jiao2021robust}, where data uncertainty is modeled with Gaussian distribution.
% Solely using spinning LiDARs for pose estimation is not ideal since registration using skewed point clouds or features will eventually cause large drift. 
% There are multiple work on fusing LiDARs with different modalities.
% Tightly-coupled systems usually offer improved accuracy
% and are presently a major focus of ongoing research [14].
% In [15], preintegrated IMU measurements are exploited for
% de-skewing point clouds. A robocentric lidar-inertial state
% estimator, R-LINS, is presented in ~\cite{qin2020lins}. R-LINS uses an
% error-state Kalman filter to correct a robot’s state estimate
% recursively in a tightly-coupled manner. Due to the lack
% of other available sensors for state estimation, it suffers
% from drift during long-during navigation. A tightly-coupled
% lidar inertial odometry and mapping framework, LIOM, is
% introduced in ~\cite{ye2019liomap}. LIOM, which is the abbreviation for
% LIO-mapping, jointly optimizes measurements from lidar and
% IMU and achieves similar or better accuracy when compared
% with LOAM. Since LIOM is designed to process all the
% sensor measurements, real-time performance is not achieved
% - it runs at about 0.6× real-time in our tests.
% In~\cite{corso2013indoor}, a backpack lidar system (BLS) has been proposed which has a wide application prospect in mapping places that LiDAR-equipped vehicles or robots cannot access to. The BLS system consist of two spinning lidar 
 % Most of the system presume that all sensors has been synchronized with an hardware-based external clock~\cite{jiao2021robust}. 
% Both ~\cite{corso2013indoor, jiao2021robust} presume the system has been hardware synchronized, and the raw cloud and the feature cloud are conjugated after relative extrinsic transformation. 
% 
% A tightly coupled LiDAR-inertial system designed for multiple LiDARs with complementary FoV is proposed in ~\cite{nguyen2021miliom}.
% 
% However, the temporal difference haven't been taken into consideration. 
% % \subsection{Multi Lidar System}
% There is no almighty and perfect sensor so far, and every sensor has its limitation. For example, the 3D spinning LiDAR has a large field of view(FoV), but the sparse characteristic of this kind of LiDAR sensor limited its performance in semantic-analyzing tasks. On the contrary, the solid-state lidar with non-repetitive scanning mode has a limited FoV but provides a denser geometry measurement within the FoV, which improves the detection of objects and details of the surrounding environment. Furthermore, due to the low update frequency,  the LiDAR sensor's performance usually suffers from fast movement as it may distort the data, so the Inertial Measurement Unit(IMU) has been widely utilized in navigation and mapping tasks.  
 % 
% 
% \subsection{Inherent Error and pointcloud undistortion} 
% To avoid the drifting along sized the Z-axis, ground points are extracted as a constraints to optimize the odometry accuracy in ~\cite{ye2019liomap}. However, for some environment, such as indoor environment and cave, collecting enough ground points are not always possible. 
% To overcome the in-homogeneous density of mobile laser scans, a feature equalizer is proposed and included in SLAM framework that seeks to balance the in-homogeneous feature points of buffered scans in a
% sliding window and make them uniformly distributed to the best possible extent ~\cite{chen2022hysteretic}.

% \red{TODO: UNDISTORTION WORKS}


% In method propsoed in ~\cite{xu2022robust} view the scan as a series of rectangular sub-region blocks, namely geometric unit, and down-weighted in losses based on the 3D point covariance estimations in ego-motion optimization. Nevertheless, the learning based ... \red{...}
% To increase the measurements density, high resolution spinning lidar(64,128 channels) are used in~\cite{shan2021robust}, or multiple low resolution spinning lidars system are introduced~\cite{chen2021backpack}. However, both methods are costly which avoid widely application. Our methods adopt the low-resolution spinning lidar and an low-cost solid-state-lidar, to enhance the environment perception ability.  
 
% Sparse methods prefer to extract geometric features from raw measurements and are, thus, supposed to have real-time performance. Recently, several following methods have employed ground planes~\cite{shan2018lego}, ~\cite{chen2020sloam}, visual detection~\cite{chen2020sloam}, good features ~\cite{jiao2021greedy}, or directly used dense scanners~\cite{lin2020loam, xu2022fastlio2} to improve the performance of sparse approaches in noisy or structureless environments. 
% To limit the computation time when more LiDARs are involved, we extract the sparse edge and planar features like LOAM. But differently, we represent their residuals in a more concise and unified way


% \subsection{Localizability Estimation}
% environment degeneracy has been explored in ~\cite{zhang2016degeneracy}, however, the proposed methods can estimate the degeneracy direction based on the information matrix but the system still cab provide a result .. 

% \begin{figure}[t] 
%     \centering 
%     % \includegraphics[width=0.45\textwidth]{fig/sauna_lio.jpg}
%     % \vspace{1em}
%      \includegraphics[width=0.5\textwidth]{fig/time_offset_bak.jpg}
%     \caption{The time offset between different sensor}
%     \label{fig:timeoffset} 
% \end{figure}

 

==> sec/03_MET_OLD.tex <==
 
% \begin{figure}[t] 
%     \centering  
%      \includegraphics[width=0.45\textwidth]{fig/livox_undistort.png}
%     \caption{Solid-state lidar motion un-distortion.(left) raw data from livox lidar. (b) corresponding point cloud after motion un-distortion}
%     \label{fig:livo_undistort} 
% \end{figure}

% \begin{figure}[t]
%     \centering 
%     % \includegraphics[width=0.45\textwidth]{fig/sauna_lio.jpg}
%     % \vspace{1em}
%     %  \includegraphics[width=0.5\textwidth]{fig/work_flow.jpg}
%      \includegraphics[width=0.5\textwidth]{fig/sub_maps.png}
%     \caption{submaps \& global maps \red{Example} from https://arxiv.org/pdf/2202.00242.pdf}
%     \label{fig:sys_overview} 
% \end{figure}
  
\section{System Overview}

To simplify the system design, we have made follow assumptions:1)  The LiDARs are synchronized at the software level. The time offset between sensors is not considered in our system 2)The extrinsic parameters between IMU and at least one LiDAR are known. In our case, we use LiDAR's built-in IMU and use the extrinsic parameter from factory settings.
%     \item  The extrinsic parameters between IMU and at least one lidar are known. In our case, we use the lidar's built-in IMU and get the extrinsic parameter from factory.
% \begin{enumerate}
%     \item The lidars are synchronized in software level, which means that the temporal latency among them cannot be ignored.
%     \item  The extrinsic parameters between IMU and at least one lidar are known. In our case, we use the lidar's built-in IMU and get the extrinsic parameter from factory.
% \end{enumerate}
 
\subsection{Overview} 
The design of our system is motivated by our previous work~\cite{li2022dataset} where solid-state LiDAR shows significant performance outdoors but failed all tests indoors. To combine the high situation awareness ability and robust performance, here we proposed  multi-modal LiDAR-inertial odometry and mapping scheme.
 In this paper, we consider a perception system consisting of multiple modal LiDARs and IMU, and LiDAR sensors are not triggered by hardware based external clock.
The pipeline of the proposed method is illustrated in Fig.~\ref{fig:sys_overview} and the hardware system is shown in  Fig.~\ref{fig:hardware_platform}. Our hardware is composed of a spinning LiDAR Velodyne VLP-16, a low-cost solid-state LiDAR Livox Horizon, and its built-in IMU.

\subsubsection{System pipeline}

The system starts with a data pre-processing module, in which IMU data are pre-integrated, extrinsic parameters between sensors are calibrated, timestamps of clouds with different starting times are aligned, the clouds from multiple LiDARs are un-distorted with IMU pre-integrated results.
        % . With the estimated transformation from IMU, the cloud evaluation part first de-skew the cloud to reduce the motion effect and equalize the distribution of the feature pointcloud in space.
After pre-processing, feature pointcloud representing plane and edge points are extracted and merged into one cloud. The merged feature cloud will be sent to the sliding window odometry module where the feature cloud will be matched against the local map. Together with pre-integrated IMU, fixed size of feature clouds and local map, six-DoF egomotions and IMU parameters are estimated and optimized by keyframe-based sliding window optimization.
% The merged points will be matched against the global map which provided pose graph back-end.
% 
% The mapping module takes selected feature cloud and pre-integrated IMU information as input. We maintain a sliding window for the feature cloud from the primary lidar and apply the optimization method on a few latest sweeps together with the feature map provided by the mapping module. For point clouds from the auxiliary lidars, the Odometry module applies frame-to-map motion estimation. 
 % 
% 
At the backend, the system maintains a global pose graph with selected keyframes. Loop closure is detected in a keyframe basis graph using ICP, and a global graph optimization is invoked to guarantee the reconstructed map is globally consistent.
% % 
% With the cloud data with its corresponding optimized pose from sliding window optimization and pose graph optimization, a global plane   map is build and processed when a new plane is detected by RANSAC method.
 
 
\subsubsection{Notation and Problem Formulation} 
 We treat IMU coordinate as the base local coordinate indicated as $()^{b}/()^{I}$. The merged cloud will be transformed to $()^{b}/()^{I}$. We use the first keyframe received by the system as the origin of the world coordinate denoted as $()^w$. 
 The coordinate of spinning LiDAR is denoted as $()^{v}$, and coordinate of solid-state LiDAR are denoted as $()^{h}$.
 We use $\mathcal{P}_{t_1}^v = \{ \textbf{p}_1^v,\textbf{p}_2^v,...\textbf{p}_n^v\}$ be the point cloud acquired at time $t_1$ with spinning LiDAR, and $\mathcal{P}_{t_2}^h = \{ \textbf{p}_1^h,\textbf{p}_2^h,...\textbf{p}_n^h\}$ be the cloud acquired at time $t_2$ with solid state LiDAR, where $\textbf{p}_i^v$ and  $\textbf{p}_j^h$ are a point in $\mathcal{P}_{t_1}^v$ and $\mathcal{P}_{t_2}^h $.
 
 % For each 3D LiDAR, we denote every channel of measurement captured by the 3D LiDAR sensor as scan \textit{C}, and denote sweep as \textit{S} which contains all the scans in one measurement. 
 We denote \textit{${\mathbb{F}_E}_k$} and \textit{${\mathbb{F}_P}_k$} as the edge and plane feature pointcloud extracted from the LiDARs’ data at time $k$. 
 % 
The transformation matrix is denoted as $\textbf{T}_a^b \in SE(3)$
which transforms a point from frame $()^a$ into the frame $()^b$. 
$\textbf{R}_a^b\in SO(3)$ and $\textbf{t}\in R^3$ are the rotation matrix and the translation vector of $\textbf{T}_a^b$ respectively. 
The quaternion $\textbf{q}_a^b$  under Hamilton notation is used, which corresponds to  $\textbf{R}_a^b$. $\otimes$ is used for the multiplication of two quaternions. $\textbf{q}_a^b$ and $\textbf{R}_a^b$ can be convert by Rodrigues formula. 
% 
With given pointcloud from multi-modal LiDAR sensor and IMU info, the state need to be optimized for keyframe $k$ are defined as (\ref{eq:frame_state}) where $\textbf{t}_k$ is the translation vector, ${\textbf{q}_k}$ represents orientation in quaternion, ${\textbf{v}_k}$ is the velocity, $\textbf{b}_{a_k}$ and $\textbf{b}_{g_k}$ are the bias vector of the accelerator and gyroscope. 
% 
\begin{equation}
 {\mathbf{X}_k} = [\textbf{p}_k, \textbf{q}_k, \textbf{v}_k, \textbf{b}_{a_k}, \textbf{b}_{g_k}] \in \mathbb{R}^3 \times \mathbb{S}^3 \times \mathbb{R}^3 \times \mathbb{R}^3 \times \mathbb{R}^3 
 \label{eq:frame_state}
\end{equation}

% \subsubsection{IMU-Centric Temporal offset Estimation}
% The time offsets between the exteroceptive sensors and the IMU are commonly exist low-cost devices due to sensor latency, clock skew, or data transmission delays~\cite{zuo2019lic}. Most existed multi-lidar sensor system assume the timestamp between multiple sensors are well synchronized. However, reliable hardware synchronization is not always available, especially for self-assembled multi-sensor platform. The objective of this process is estimate the time offset between different sensor, which is crucial for tightly-coupled lidar inertial methods.

% As different lidar system may adopt different time-stamp as ~\ref{fig:timeoffset}, we assume the delay between the sensor and the computer are fixed, and the data are published at a fixed frequency. As the clock may different, so we adopt the computer time of first received frame as the base stamp of each message, and the followed message timestamp will be compute based on this stamp and time difference. Since, then all the message time will be transformed to the IMU centric system.

% Based on the result from ~\cite{yang2019degenerate}, one-axis rotation perform better in terms of time offset estimation.
 
% \blue{
% To merge two pointcloud, we adopt a spatio-temporal calibration, split-and-merge methods similar to ~\cite{chen2021backpack}.The individual timestamp of each point from lidars can be obtained from Velodyne ROS driver and Livox pointcloud.That is, each point in Horizon is first split according to the starting timestamps of the closet point from VLP-16 in the point sequence. Thereafter, the split points of point from Horizon are transformed by $T_{ex}$, and merged into Velodyne Pointcloud that shares the same time domain. 
% N ote that the extrinsic parameter $T_{ex}$ is obtained offline, but the “split-and-merge” is processed online.
% }



% \subsection{IMU MAP initialization}
% Based on the IMU preintegration method proposed in ~\cite{qin2018vins}
% the motion distortion of the point cloud is compensated using IMU preintegration with constant velocity model.Inspired by ORB-SLAM3~\cite{campos2021orb}, a maximum a posteriori (MAP) estimation method is adopted to jointly initialize IMU biases, velocities, and the gravity direction. This method doesn't need a careful initialization process. The system can be initialized with an arbitrary motion. This method takes into account sensor uncertainty, which obtains the optimum in the sense of maximum posterior probability.

  

\subsection{Pre-processing}

\subsubsection{Spatial-temporal Calibration and Initialization} 
\label{sec:st_cali}

% To obtain reliable pose estimation, sensors need to be carefully calibrated and initialized. 
As the extrinsic parameter between IMU and one LiDAR is known, so here we focus on calibrating the extrinsic parameters between two LiDARs. We assume the sensor platform is stationary during the extrinsic calibrations process.
% In this part, we introduce the calibration and initialization methods we utilized in proposed framework.
% To get transformation between the reference lidar coordinates and the coordinates of each lidar via optimization approach.    
% solid-state lidar was treated as a reference frame during the calibration process. 
As solid-state LiDAR with the non-repetitive pattern is able to obtain more details from the environment within the FoV, therefore, we integrated $n$ consecutive frames(e.g., ten) to new point cloud $\mathcal{P}^h_{t_1\sim t_n}$ for the calibration process. Let $\mathcal{P}^v_{t_m}$ be one cloud data obtained at $t_m \in (t_1, t_n)$ from spinning LiDAR.
% 
Generalized Iterated Closest Point (GICP)\cite{segal2009gicp} method is employed to caculate the relative transformation matrix $\textbf{T}_{v}^h$ between $\mathcal{P}^h_{t_1\sim t_n}$ and $\mathcal{P}^v_{t_m}$ from the overlapped region. The extrinsic calibration results with data collected from a classroom environment are shown in Fig. \ref{fig:extrin_cali}. As the transformation matrix $\textbf{T}_{h}^i$ between IMU and one LiDAR given by the factory, we can get $\textbf{T}_{v}^i$ by
    $\textbf{T}_{v}^i  = \textbf{T}_{v}^h * \textbf{T}_{h}^i$. 
% Then, all extrinsic parameters between sensors are known.

We consider a system that LiDARs are not triggered with the external clock(e.g. GNSS) like~\cite{jiao2021robust}, each cloud $\mathcal{P}^h$ and $\mathcal{P}^v$ are collected at different starting timestamps. To merge clouds into one combined cloud $\mathcal{P}^m$, we need to align the starting timestamp and ending timestamp.  
 % 
We adopt a split-and-merge methods similar to ~\cite{chen2021backpack}.The individual timestamp of $p_i^h \in \mathcal{P}^h$ and $p_i^v \in \mathcal{P}^v$ can be obtained from sensors driver. If timestamp for point $p_i^v \in \mathcal{P}^v$ is not available, it also can be calculated by orientation difference~\cite{zhang2014loam}. 
% 
When a new cloud $\mathcal{P}^h_{t_k}$ received at time ${t_k}$, we put all points $p_i^v \in \mathcal{P}^h_{t_k}$ to a queue $\mathbb{Q}^h$ which ordered by timestamp. When a new cloud $\mathcal{P}^v_{t_m}$ received at time $t_m$, we first get its start time $t_{m_s}$ and end time $t_{m_e}$, then all points in  $\mathbb{Q}^h$ which timestamp $t_i < t_{m_s}$will be dropped, and $t_i \in (t_{m_s}, t_{m_e})$ will be popped to a new frame $\mathcal{P}^h_{t_m}$ which share the same time domain with $\mathcal{P}^v_{t_m}$.
%  
 \subsubsection{IMU Initialization and Preintegration}
 
The IMU sensor output angular velocity and acceleration measurements are defined as $\tilde{\omega}_t$ and $\tilde{\mathbf{a}_t}$ using equations. \ref{eq:raw_ang} and \ref{eq:raw_acc}: 
\begin{equation}
\label{eq:raw_ang}
    \boldsymbol{\omega}_t =  \boldsymbol{\omega}_t + \mathbf{b}_t^{ \boldsymbol{\omega}} + \mathbf{n}_t^{ \boldsymbol{\omega}}
\end{equation}
\begin{equation} 
\label{eq:raw_acc}
    \tilde{\mathbf{a}_t} = \mathbf{R}_t^{WL}( \mathbf{a}_t - \mathbf{g}) + \mathbf{b_t}^{\mathbf{a}} + \mathbf{n_t}^{\mathbf{a}}
\end{equation}
Where $ \mathbf{b}_t$ is the measurement bias and $\mathbf{n}_t$ is white noise. 
$\mathbf{R}_t^{LW}$ is the rotation matrix from World coordinate $()^L$ to local coordinate $()^W$, $\mathbf{g}$ is the  gravity vector in world coordinate. Based on the raw measurement $\boldsymbol{\omega}_t$ and $\tilde{\mathbf{a}_t}$ , we can infer the motion of the robot as follows: 
\begin{equation} 
\label{eq:imu_pose}
\begin{aligned} 
\mathbf{p}_{t +  \Delta{t}} =  \mathbf{p}_t + &\mathbf{v}_t \Delta{t} + \frac{1}{2}\mathbf{g}\Delta{t}^2 +   \\
    &\frac{1}{2} \mathbf{R}_t(\mathbf{\hat{a}}_t - \mathbf{b}_t^{\mathbf{a}} - \mathbf{n}_t^{\mathbf{a}}) \Delta{t}^2
\end{aligned}
\end{equation} 
\begin{equation}  
\label{eq:imu_velo}
\mathbf{v}_{t +  \Delta{t}} = \mathbf{v}_t + \mathbf{g}\Delta{t} +   \mathbf{R}_t(\mathbf{\hat{a}}_t - \mathbf{b}_t^{ \mathbf{a}} - \mathbf{n}_t^{\mathbf{a}}) \Delta{t}
\end{equation} 
\begin{equation}
 \label{eq:imu_quat}
 \begin{aligned}
\mathbf{q}_{t +  \Delta{t}} &= \mathbf{q}_t \otimes \mathbf{q}_{\Delta{t}} \\ 
&= \mathbf{q}_t \otimes  
 \begin{bmatrix}
exp( \frac{1}{2}  \Delta t ( \tilde{ \boldsymbol{\omega}}_t - \mathbf{b}_t^{\boldsymbol{\omega}} - \mathbf{n}_t^{\boldsymbol{\omega}}))
\\
1
\end{bmatrix}
\end{aligned}
\end{equation}

Where the  $\mathbf{p}_t, \mathbf{v}_t$ and $\mathbf{q}_t $ are the estimated position,velocity and orientation in quaternion at time $t$, $\mathbf{p}_{t +  \Delta{t}}, \mathbf{v}_{t +  \Delta{t}}$ and $ \mathbf{q}_{t +  \Delta{t}}  $ are the estimated state at time $t+\Delta{t}$.
We apply the IMU preintegration method proposed in ~\cite{qin2018vins}. The relative motion between two timestamp $\Delta{\mathbf{V}}, \Delta{\mathbf{P}}, \Delta{\mathbf{Q}}$ can be caulated based on equations \ref{eq:imu_pose}$\sim$\ref{eq:imu_quat} and will be used for initial guess in ~\ref{sec:sliding_win}.
 
% \subsubsection{Plane based Motion un-distortion}
% \blue{TODO: Decide if we keep this! 
% As for solid-state lidar featuring non-repetitive scanning pattern, we can 
%  \begin{equation}
% \begin{aligned} 
%    {\min_{\mathbf{x}^w, \varphi } } \left \{ \sum_{i=1}^{m} \left ( \mathfrak{D}_e \left ( \mathbf{x}^w, \mathbf{p}_i^{\mathrm{C}}, \mathbb{M}^w \right )   \right )^2   
%    % +   \sum_{j=1}^{N} \left ( \mathfrak{D}_e \left ( \mathbf{x}^w, \mathbf{p}_j^{\mathrm{C}}, \mathbb{M}^w \right )   \right )^2  
%    + \sum_{k=1}^{k} \left ( \mathfrak{D}_e \left ( \mathbf{x}^w,  \varphi, \mathbf{p}_k^{\mathrm{C}}, \mathbb{M}^{\mathfrak{p}} \right ) \right )^2 \right \}  
% \end{aligned}
%  \end{equation}
% Here we only match the edge feature agianst global edge feature map, 
% instead of matching against feature map, we also consider the global plane map where the distortion parameters can be optimized.
% } \\ 
 
\subsection{Multi-modal LiDAR Pose Estimation}  

\subsubsection{Union Feature Extraction}

For computing efficiency, feature extraction is essential for the SLAM system. We focus on extracting the general features that exist in different modal lidars and can be shared in the optimization process. 
Here we extract feature points based on~\cite{li2021towards} that selects a set of feature points from measurements according to their continuous and surface normal vector. We extend the method and adapt it to both spinning and solide-state-lidar.
The set of extracted features consists of two subsets: plane points $\mathbb{F}_P$ and edge points $\mathbb{F}_E$. By checking the continuity, the edge feature included two types of points $\mathbb{F}_{E_l}$ and $\mathbb{F}_{E_b}$ where $\mathbb{F}_{E_l}$ represents the line feature where two surface meets, and $\mathbb{F}_{E_b}$ represents breaking points where plane end.  
 
Let $\mathcal{P}^v_t $ be the pointcloud acquired at time $t$ from spinning lidar, $\mathcal{P}^h_t$ be the point cloud acquired from solid-state lidar at the same time domain after temporal alignment. 
% Velodyne feature points extraction.
If the channel number of each point $p_v \in \mathcal{P}^v_t$ is unavailable, then We first projecte points in $\mathcal{P}^v_t$ onto a range image based on the horizontal and vertical angle w.r.t. the origin. Each row represent data from one channel of the spinning lidar. Then the points are divided into $N$ subsets $\{\mathbf{L}^v_i\}_{i\in N}$ where $N$ is the total channel numbers of spinning lidar.
For point cloud $\mathcal{P}^h_t$, we divide the point based on line number which can  obtained from Livox ROS driver~\footnote{\url{https://github.com/Livox-SDK/livox\_ros\_driver}}. Similarly, we first divided the points into $M$ subsets $\{\mathbf{L}^h_i\}_{i\in M}$ where $M$ is the total line numbers of solid-state lidar. The points in each ${\mathbf{L}^v_{i}}_{i\in N}$ and ${\mathbf{L}^h_{i}}_{i\in M}$ are ordered by timestamp.
% 
% 
For each subset $\mathbf{L}^v_i$ in $\{\mathbf{L}^v_i\}_{i\in N}$ and $\mathbf{L}^h_j$ $\{\mathbf{L}^h_j\}_{j\in M}$, we first extract the continues points ${\mathcal{P}^v_i}_C$ and ${\mathcal{P}^h_j}_C$ by checking the depth difference with its neighbour points. If the  depth difference between the point in $\mathbf{L}^v_i$ or $\mathbf{L}^h_j$ and nearest neighbor points within same subset are smaller the the depth threshold $d_{th}$, then the point are added to continuous points subset ${\mathcal{P}^h_i}_C$ or ${\mathcal{P}^v_j}_C$.
% 
Then we follow the feature extraction methods in~\cite{chen2021backpack}, where a scatter matrix $\boldsymbol{\Sigma}$ is calculated based on neighbor points. By analysing the two largest eigenvalue $\lambda_1$ and  $\lambda_2$ of $\boldsymbol{\Sigma}$, the plane points are detected and labelled as plane,  the point where two plane meet is labeled as corner features, the points where one plane ends and neighboring with an discontinuous points are labeled as break points. We merge the corner points and break points together and use it as edge feature points.
After this process, plane feature points ${\mathbb{F}^h_P}_{t}$ and  ${\mathbb{F}^v_P}_{t}$, edge feature points  ${\mathbb{F}^h_E}_{t}$ and ${\mathbb{F}^v_E}_{t}$ are extracted.
% 
We show extracted feature points in office room environment in Fig.~\ref{fig:feature_pts} 
% 
\subsubsection{Feature Clouds Merging}

Instead of keep two different system state $\textbf{X}_t$ for clouds $\mathcal{P}_t^h$ and  $\mathcal{P}_t^v$ , we merge the same type of feature point cloud into one frame and use one system state . As the cloud $\mathcal{P}_t^h$ from solid-state lidar can be blocked near by objective, or all points lie on single plane(e.g., wall) in indoor environment, this make most of points in ${\mathbb{F}^h_P}_{t}$ belong to single plane and insufficient ${\mathbb{F}^h_E}_{t}$ can be extracted. 
In this case, we treat the $\mathcal{P}_t^h$ as "bad frame" which corresponding feature cloud will not be added to union feature cloud ${\mathbb{F}^i_{E}}_t$ and ${\mathbb{F}^i_{P}}_t$ to make the system more efficient.
To detect "bad frame", We first remove the point in ${\mathbb{F}^h_P}_{t}$ and  ${\mathbb{F}^h_E}_{t}$ that close to the origin of sensor(e.g., 2m), and then check the amount $n_e$ of edge point in feature cloud ${\mathbb{F}^h_{E}}_t$. If $n_e$ smaller then the edge feature threshold $\tau_e$(e.g., 100), then the cloud $\mathcal{P}_t^h$ is treated as "bad frame". 
% 
If no "bad Frame" detected, we transform all feature cloud  ${\mathbb{F}^h_P}_{k}$,  ${\mathbb{F}^v_P}_{t}$,  ${\mathbb{F}^h_E}_{t}$ and ${\mathbb{F}^v_E}_{t}$ to $()^i$ coordinate and merge them to one unified feature clouds ${\mathbb{F}^i_{E}}_k$ and ${\mathbb{F}^i_{P}}_k$ with extrinsic transformation matrix $\textbf{T}_v^i$ and $\textbf{T}_h^i$ caculated in sec. \ref{sec:st_cali} by
$$ \mathbb{F}^i_{E}  = \textbf{T}_v^i * \mathbb{F}_{E}^v + \textbf{T}_h^i * \mathbb{F}_{E}^h , \mathbb{F}^i_{P} = \textbf{T}_v^i * \mathbb{F}_{P}^v + \textbf{T}_h^i * \mathbb{F}_{P}^h.$$ 
If $\mathbb{P}_t^h$ is "bad frame", then  
$ \mathbb{F}_{E}^i  = \textbf{T}_v^i * \mathbb{F}_{E}^v$ and $ \mathbb{F}_{P}^i = \textbf{T}_v^i * \mathbb{F}_{P}^v.$
 % 
% 
The union feature clouds $\mathbb{F}_{E}^i$ and $\mathbb{F}_{P}^i$ will be down-sampled before sending them into sliding window optimization module.
 
% % Then with the continuous points in $\mathbf{P}_C$, 
% For each continuous points subset, we calculate it's left neighbors curvature $\mathcal{C}_l$ and right neighbor curvature $\mathcal{C}_r$ by: 
%  \begin{equation}
%      c = \frac{1}{|S|.||d_i||} || \sum_{j \in S, j \neq i}(d_j - d_i)||
%     \label{eq:curv_cacu}
%  \end{equation}
% where $S$ is a set of continuous points belong to ${\mathcal{P}^h_i}_C$ or ${\mathcal{P}^v_j}_C$, $d$ represent the Euclidean distance from lidar origin to current point. 
% % 
% Then the points are divided into edge Feature and plane Feature by a given edge feature threshold $\mathcal{C}_{e_{th}}$ and plane feature threshold  $\mathcal{C}_{p_{th}}$, where a the curvature difference larger than $\mathcal{C}_{e_{th}}$ then it belong to edge feature set $\mathbb{F}_{E}$, smaller than $\mathcal{C}_{p_{th}}$ then it belong to plane feature set $\mathbb{F}_{P}$.
 

 % 
 
 % As sliding window based optimization method require huge power and computation resource, to improve the efficiency of the system, only the feature clouds are sent to fix-laged sliding window to conduct Bundle adjustment. Feature cloud auxiliary lidar only conduct the frame-to-map registration. 
% To get accurate pose estimation, we conduct sliding window optimization with feature points and pre-integrated IMU. 
 
% \subsubsection{Feature based scan-to-Map registration} 
% Given a feature pointcloud $\{\mathbb{F}_{E}^k, \mathbb{F}_{P}^k\}$ and a pointcloud feature map $\mathbf{M}$, the registration problem can be formulated as solving a non-linear least square problem.
% Tightly-coupled lidar-inertial fusion via sliding window optimization has been well illustrated in~\cite{li2021towards}.
% Here we conduct scan to local registration to estimate position.

% For the principle lidar data, we perform a light weight, feature based scan-to-map registration. Current pose $X^w$is estimated by minimizing 
% % $$  
% % { \tilde{X^w}} = argmin \{  \sum_{k=1}^{m} E_{Lidar}(\check{X^w}) +  \sum_{k=1}^{n} E_{Imu}(\check{X^w}) \}$$ 
%  % 
% % 
% $$\min_{\mathbf{x}^w} \left \{  \sum_{i=1}^{m} \left ( \mathfrak{D}_e \left ( \mathbf{x}^w, \mathbf{p}_i^{\mathrm{C}}, \mathbb{M}^w \right )   \right )^2  + \sum_{J=1}^{N} \left ( \mathfrak{D}_e \left ( \mathbf{x}^w, \mathbf{p}_j^{\mathrm{C}}, \mathbb{M}^w \right ) \right )^2 \right\} $$

 
% which incorporate all the edge and plane correspondences between current scan and global feature map M. 
% https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=9392274
   
% \subsubsection{Feature cloud  selection}
% As both feature points from both lidars has been registered to local map, we merge the feature clouds into one single frame $()^b$, this can reduce the parameters that need to be optimized in back-end fusion and reduce the computing burden. 
% $$ \mathbb{F}_{c_e} =  \mathbb{F}_{v_e} + ( \mathbb{R}* \mathbb{F}_{l_e} + \mathbb{T} )$$
% $$ \mathbb{F}_{c_p} =  \mathbb{F}_{v_p} + ( \mathbb{R}* \mathbb{F}_{l_p} + \mathbb{T} )$$
% As the inherited mechanism difference from lidar sensors, feature points are detected in different cloud distribution. In order to maintain one feature map that can be used for different modal lidar, we merge two separated feature cloud into one cloud with feature selection process. As solid-state lidar has higher resolution within FoV, therefor all feature points within same FoV will be updated based on nearby feature points from solid-state lidar


% \subsubsection{Lidar Odometry Factor} 
% \begin{equation}
% \begin{aligned} 
%   \sum_{k=1}^{m} E_{Lidar}(\check{X^w}) =      \sum_{i=1}^{m} & \tilde{e}_{i} (D_e(\check{X_k^w}, \check{p_{k,i}^w})) ^2    \\   + & \sum_{j=1}^{m}  \tilde{e}_{j} (D_p(\check{X_k^w}, \check{p_{k,j}^w})) ^2  
% \end{aligned}
% \end{equation}
%  Here, $D_e$ and $D_p $  are the point-to-edge and point to plane metrics with correspondences feature points in feature map. The local map is updated with the given optimized pose as the window slides. It worth to notice that the lidar odometry here can generated from different modal of lidars.
 
% \subsubsection{Pre-integrated IMU Factor}
% The error term for IMU provide the motion constraints between keyframe into the sliding window. We adopt the pre-integrated inertial methods to adopt relative motion measurement $\Delta r = ( \hat{\alpha}_j^I, \hat{\beta}_j^I, \hat{\gamma}_j^I ) $ between two consecutive key-frames $k$ and $k+1$ as ~\cite{qin2018vins}. The error term is defined as 

% \begin{equation} 
% e_{ij} = \begin{bmatrix}  \alpha_{j}^w 
% \\  \beta_{j}^w
% \\  \gamma_{j}^w
% \\ \mathbf{b}_{aj} 
% \\ \mathbf{b}_{wj}  
% \end{bmatrix}
%  \ominus 
% \begin{bmatrix} \mathbf{P}_{j}^w - \mathbf{P}_{i}^w + \frac{1}{2}\mathbf{g}\delta t^2 - \mathbf{V}_i^w \delta t 
% \\ \mathbf{V}_{j}^w - \mathbf{V}_{i}^w - \mathbf{g} \delta t  
% \\ {\mathbf{q}_{i}^{w}}^{-1}  \otimes q_j^w
% \\ \mathbf{b}_{ai} 
% \\ \mathbf{b}_{wi} 
% \end{bmatrix}
% \end{equation}

% Where rotation matrices $R$ and Hamilton quaternions $q$ are used to represent rotation. $\mathbf{P}_{i}^w,\mathbf{V}_{i}^w,$ and $\mathbf{q}_{i}^w$ are translation, velocity, and rotation from the body frame to the world frame. $\mathbf{g}$ is the gravity vector in the world frame. $\mathbf{b_a}$ and bw are accelerometer bias and gyroscope bias respectively. $\otimes$ is the minus operation on the IMU residuals.The accelerometer bias error and gyroscope bias error are jointly optimized in the graph.
 
% The nonlinear least square problem in ~\ref{eq:slide_error} can be solved using typical solvers, e.g., the trust region method. Constrained by the optimized keyframes, regular LiDAR frames in between are obtained via local graph optimization. After the fusion window slides over, the newly obtained LiDAR poses are inserted into a global pose graph with only keyframe feature maps maintained for mapping purpose.

 

% % Loop closure detection
% To detect potential loop closures, we search in the global graph, e.g., in a radius of 10 m, to find keyframe nodes that are spatially close but with enough temporal distance (e.g., 20 keyframes). An ICP is performed between the current feature scan and the candidate feature map, from which a fitting score is computed for loop closure detection. Once confirmed, a global pose graph optimization is invoked by imposing the constraint from the ICP. As depicted in Fig. 2, the keyframe local map M˘ w at backend is then updated by corrected poses to further incorporate the LiDAR constr


% \subsection{Uncertainty Aware Loop Closure Detection}
% \blue{ sub-maps with localization uncertainty in graph optimization} 

\subsubsection{Key\-frame Selection \& Un\-distortion}
\label{sec:sliding_win}

Given feature pointcloud and preintegrated IMU within same time domain 
${\mathbb{F}^i_E}_k, {\mathbb{F}^i_{P}}_k , {\mathbb{I}^i_{preg}}_k $ and a pointcloud feature map $\mathbb{M}^w_k$ in world coordinate, the registration problem can be formulated as solving a non-linear least square problem.
% 
% estimated parameters
% For each keyframe in sliding windows, the state that need to be estimated of each key-frame are defined as~\ref{eq:frame_state}, where $\tilde{p}$ is the position, $\tilde{q}$ orientation in quaternion, $\tilde{v}$ is the velocity, $ \tilde{b_a}$ and $ \tilde{b_a}$ are the IMU bias of the accelerator and gyroscope. 
% % 
% \begin{equation}
%  \tilde{\mathbf{X}} = [\tilde{p}, \tilde{q}, \tilde{v}, \tilde{b_a}, \tilde{b_g}] \in \mathbb{R}^3 \times \mathbb{S}^3 \times \mathbb{R}^3 \times \mathbb{R}^3 \times \mathbb{R}^3 
%  \label{eq:frame_state}
% \end{equation}
% 
% The initial guess.
The initial guess of state $\textbf{X}^w$ are estimated by:
$$ {\tilde{\mathbf{p}}}_k=  {\bar{\mathbf{p}}_{k-1}}+  {\ {\bar{\mathbf{q}}}_{k-1}}*\Delta{\mathbf{P}}_{k-1}^k$$
$$ \ {\tilde{\mathbf{q}}}_k= {\ {\bar{\mathbf{q}}}_{k-1}}*\Delta{ \mathbf{Q}}_{k-1}^k,   {\mathbf{\tilde{b_g}}_{k}} =  {\ { {\mathbf{\bar{b_g}}}}_{k-1}}$$
$$ \ {\tilde{\mathbf{v}}_k} =  {\bar{\mathbf{v}}_{k-1}}+ \ {\bar{\mathbf{q}}_{k-1}}*\Delta{\mathbf{V}}_{k-1}^k, \ {\tilde{\mathbf{b_a}}}_{k} = {\bar{\mathbf{b_a}}_{k-1}}$$
As the sliding window optimization is a relative heavy process, therefore, maintain the sparsity of the frames in window can significantly affect the real-time performance. Here we check the IMU drift during the time interval of two consecutive key frames, and select the frame as keyframe if the orientation difference is higher than certain degree (e.g., 30\degree) or the time difference between current frame and last keyframe larger then certain time (e.g., 2 seconds).
Then each point in selected keyframe will be un-distorted with $\Delta{Q}$ and $\Delta{P}$ provided by IMU pre-integration. 
% 
Each keyframe contains deskewed feature clouds ${\mathbb{F}^i_{E}}_k$ and ${\mathbb{F}^i_{P}}_k$, pre-integrated IMU ${\mathbb{I}^i_{preg}}_k$, and initial guess of state ${\tilde{\mathbf{X} }}^w_k \sim [\tilde{\mathbf{p}}_k, \tilde{\mathbf{q}}_k, \tilde{\mathbf{v}}_k, {\tilde{\mathbf{b}_a}_k}, {\tilde{\mathbf{b}_g}_k}]$ which will be optimized by sliding window optimization.
 
\subsubsection{Sliding Window Optimization}
 In this paper, we follow keyframe based tightly coupled lidar-inertial sliding window optimization strategy in~\cite{li2021towards}. The merged feature points  ${\mathbb{F}^i_{E}}_k$ and ${\mathbb{F}^i_{P}}_k$ of keyframe $k$ are treated as feature clouds that extracted from single lidar sensor as in~\cite{li2021towards}.
 % https://arxiv.org/pdf/2010.13150.pdf QQ: borrowed from here
 % 
 We build a window with $\tau$ consecutive keyframes where the states need to be optimized for each frames are $\tilde{\textbf{X}^w} = [\tilde{\textbf{X} }^w_1,\tilde{\textbf{X} }^w_2,...,\tilde{\textbf{X} }^w_{\tau}]$. The optimal state can be obtained by minimizing function:
% 
\begin{equation}
% \begin{aligned}
 % \tilde{\textbf{X}} = 
 \min_{ \tilde{\textbf{X}}} \{  || \mathbb{D}_{prior}(\tilde{\textbf{X}^w})||^2  \\ +  \sum_{k=1}^{\tau} \mathbb{D}_{L}(\tilde{\textbf{X}^w_k}) +  \sum_{k=1}^{\tau} \mathbb{D}_{I}(\tilde{\textbf{X}^w_k}) \} 
  \label{eq:slide_error}
% \end{aligned}
\end{equation}
% 
Where $||\mathbb{D}_{prior}(\tilde{\textbf{X}^w})||^2 $ represents the prior residual term which is generated by marginalizing oldest frames before the current window via Schur-complement~\cite{qin2018vins},$\mathbb{D}_{I}(\tilde{X^w})$ represents the pre-integrated IMU terms as defined in~\cite{li2021towards}.$ \mathbb{D}_{L}(\tilde{\textbf{X}^w_k})$ is lidar term defined as (\ref{eq:lidar_term}).
\begin{equation}
\sum_{a=1}^{m}(\mathbb{D}_e(\textbf{X}^w_k, \textbf{p}^i_{k,a}, \mathbb{M}^w_k))^2 + \sum_{b=1}^{n}  (\mathbb{D}_s(\textbf{X}_k, \textbf{p}^i_{k,b}, \mathbb{M}^w_k))^2
\label{eq:lidar_term}
 \end{equation}
$\mathbb{D}_e$ is the point-to-edge  residual term defined as (\ref{eq:edge_cost}) and $\mathbb{D}_s$ point-to-plane residual term defined as (\ref{eq:plane_cost}). 
%  \tilde{v_{e,i}}  \tilde{v_{s,j}} 
% $\tilde{v_e}$ and $\tilde{v_s}$ denote normalized weights among feature correspondences of each type.
\begin{equation}
    \mathbb{D}_e( \textbf{X}^w,\textbf{p}^i,\mathbb{M}^w)) = \frac{||( \textbf{p}^w - 
 \boldsymbol{\acute{e}^w}  )\times( \textbf{p}^w -  \boldsymbol{\grave{e}^w}   ) ||}{ || \boldsymbol{\acute{e}^w} -  \boldsymbol{\grave{e}^w}||}
 \label{eq:edge_cost}
\end{equation}
% 
\begin{equation}
    \mathbb{D}_s( \textbf{X}^w,\textbf{p}^I,\mathbb{M}^w)) =  | \textbf{n}_s^T\textbf{p}^w + 1/|| \textbf{n}_s |||  
\label{eq:plane_cost}
\end{equation}
$\textbf{p}^i$ represent a feature point belong to ${\mathbb{F}_{E}}_k, {\mathbb{F}_{P}}_k$, 
We have $\textbf{p}^w = \textbf{R(q)}\textbf{p}^i + \textbf{t}$ that represent the scan point $\textbf{p}^i$ at local frame $()^i$ is transformed to world frame $()^w$ by state info $[\textbf{q}, \textbf{t}]$ in $\textbf{X}^w$. 
$\boldsymbol{\grave{e}^w}$ and $\boldsymbol{\acute{e}^w}$ are two closest corresponding edge feature points on feature map $\mathbb{M}^w$ and $\textbf{n}^w_s$ is the plane normal vector that is calculated by neighobors plane feature points in $\mathbb{M}^w$ cloud.
% 
 We solve the non linear equation (\ref{eq:slide_error}) with Ceres Solver~\cite{ceressolver}.
To main global consistency, we also maintain a pose-graph with optimized states $\textbf{X}^w$ and pre-integrated IMU as constraints.
% % The fusion window usually covers several selected key-frames. As the window slides,  
%  % 
% And the optimial keyframe states are obtained by minimizing~\ref{eq:slide_error}, where  $E_{prior}(\check{X^w})$ denotes the prior residual factor that are marginalized out via Schur-complement~\cite{qin2018vins}. $ E_{Lidar}(\check{X^w})$ and $E_{Imu}(\check{X^w})$ are the keyframe Lidar odometry and IMU estimation error terms.
% % 
% \begin{equation}
% \begin{aligned}
% { \tilde{X^w}} = argmin \{ &|| E_{prior}(\check{X^w})||^2  \\ +  &\sum_{k=1}^{m} E_{Lidar}(\check{X^w}) +  \sum_{k=1}^{m} E_{Imu}(\check{X^w}) \}
%   \label{eq:slide_error}
% \end{aligned}
% \end{equation}
% % 
% where $E_{prior}(\check{X^w})$ is the prior items from marginalization. $ E_{Lidar}(\check{X^w})$ is the residual of the relative lidar constraints and $E_{Imu}(\check{X^w})$ is the residual of the IMU constraints. The cost function in the form of a non-linear least square can be solved by the Gauss-Newton algorithm. We use Ceres Solver to solve the problem.
 
%  \subsubsection{Degenerate Environment detection}
% One common challenging situation for solid-state lidar is part or all of its FoV is blocked by near objects that cause insufficient features point. Due to the low vertical resolution, the performance of scan to map matching with low-cost spinning lidar will degenerate~\cite{ye2019liomap} in tunnel or corridor environment. 
% % The objective of this process is to detect these challenge environment, 
%  % 
% Inspired by the localizability estimation in~\cite{zhen2019localizability}, we estimate the localizability with $\mathbb{F}^k_p$ from lidars with equation~\ref{eq:local_ability}
% % 
% \begin{equation}
%     \mathit{L}(x, R, \rho_i) = n_i^T( x + rR_i\rho_i) + d_i % = 0
%     \label{eq:local_ability}
% \end{equation}
% Where$(x,R)\in (\mathbb{R}^3, \mathit{SO}(3))$ denotes the robot position and orientation, and $i\in \{1,2,... m\}$ is the point index in the laser scan. $(n_i, d_i) \in (\mathbb{R}^3, \mathbb{R})$ encodes the normal vector and distance which is estimated by fitting a local plane to the neighboring points.  $r_i \in \mathbb{R}^3$ is the unit range vector represented in the robot body frame and $\rho_i \in \mathbb{R}$ is the range value.
% % Eqn. ~\ref{equ:local_ability} describes a simple fact that the scanned points should align with the map when the robot is localized. 



==> sec/04_EXP_OLD.tex <==
 

 \begin{figure}[t]
    \centering  
     \includegraphics[width=0.42\textwidth]{fig_iros/platform2.png}
     % \includegraphics[width=0.4\textwidth]{fig/platform.png}
    \caption{Hardware platform is composed of Livox Horizons lidars with its built-in IMU and Velodyne VLP-16 lidar, and other sensor is not used in our experiment. The whole platform is mounted on a moving ground vehicle.}
    \label{fig:hardware_platform} 
\end{figure}
 

% \begin{table}[t]
%     \centering
%     \caption{ Dataset Details} 
%     \begin{tabular}{@{}ccccc@{}}  
%     \toprule 
%         Dataset     & Environment  & Scans number & Duration  & Trajectory    \\[0.5ex]
%      \midrule     
%         room01      & small office      & XXX & XXX & XXX  \\  [0.5ex] 
%         corridor01    & Long corridor   & XXX & XXX & XXX  \\  [0.5ex] 
%         corridor02    & Large Hall      & XXX & XXX & XXX  \\  [0.5ex] 
%         Hall01      & Forest Short      & XXX & XXX & XXX  \\  [0.5ex]
%         % Forest02    & Forest Long       & XXX & XXX & XXX  \\ 
%     \bottomrule 
%     \end{tabular}    
%     \label{table:data_details}
% \end{table} 


% \begin{figure*}[t]
%     \centering  
%      \includegraphics[width=0.9\textwidth]{fig/hall_map_plot.png}
%     \caption{The map results of sequence Hall. Our proposed methods show smallest error when return to the start point \red{TODO: 1) add more SLAM 2) add distortion difference}}
%     \label{fig:hall_map} 
% \end{figure*}

 

 
 

% \begin{figure}[t]
%     \centering   
%     % \includegraphics[trim={0cm 5cm 0cm 0cm},width=0.5\textwidth]{fig/map_detail_comp.pdf}  
%     \begin{subfigure}{0.5\textwidth}
%         \includegraphics[width=\textwidth, height=0.4\textwidth]{fig/trajectory.png}
%         \caption{The trajectory result comparison in 3D.\red{TMP}}
%     \end{subfigure}
%     \begin{subfigure}{0.5\textwidth}
%         \includegraphics[width=\textwidth, height=0.45\textwidth]{fig/trajectory_xyz.png}
%         \caption{The trajectory result comparison in X,Y,Z axis separately.\red{TMP}}
%     \end{subfigure} 
%     \begin{subfigure}{0.5\textwidth}
%         \includegraphics[width=\textwidth, height=0.45\textwidth]{fig/ape_error_plot.jpg}
%         \caption{Ape error of our proposed method (evoTUMVeloLIO) and lego loam.\red{TMP}}
%     \end{subfigure} 
% \end{figure}
  % 
 \begin{figure*}
  \hfill
     \centering 
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{fig_iros/map_details_0.png}
         \caption{Map results generated by our methods in HVI mode.}
         \label{fig:map_details_a}
     \end{subfigure}
        % \hfill
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{fig_iros/map_details_1.png}
         \caption{Map results generated Fast\_LIO in VI mode.}
         \label{fig:map_details_b}
     \end{subfigure} 
     \caption{Map details comparison on office room dataset sequence. The points color represent the reflectivity provided from raw sensor data.The point size is 1 centimetre and transparency is 0.
     05. The middle two column show the zoom-in view of the shelf (top) and TV(botom).}
     \label{fig:map_comp}
     \hfill
\end{figure*} 
\section{Evaluation}\label{sec:evaluation}

\subsection{Sensor Configuration and Implementation} 
 
We implement the proposed multi-modal multi-lidar-inertial odometry and mapping system in C++ with ROS melodic environment that can be shared in the robotic community. The system shown in Fig.~\ref{fig:sys_overview} is structured in four nodes: preprocessing, feature extraction, scan registration, and graph optimization. The factor graph optimization is maintained by GTSAM 4.0~\cite{dellaert2012factor}, and non-linear optimization is performed by Ceres Solver 2.0~\cite{ceressolver}.
% 
The framework proposed in this paper is validated using datasets gathered by Velodyne VLP-16 and Livox Horizon 3D lidars. The VLP-16 measurement range is up to 100m with an accuracy of \textpm\,3cm. It has a vertical FoV of 30\textdegree(\textpm\,15\textdegree) and a horizontal FoV of 360\textdegree. The 16-channel sensor provides a vertical angular resolution of 2\textdegree and The horizontal angular resolution varies from 0.1\textdegree to 0.4\textdegree. For solid-state lidar, we selected Livox Horizon, which is designed  with an FoV of 81.7\textdegree\,\texttimes\,25.1\textdegree. Horizon was scanning at 10\,HZ and reaches a similar but more uniform FoV coverage compared with typical 64-line mechanical LiDARs.  
The extrinsic parameter between Horizon and its built-in IMU is provided by factory instruction. The sensors are connected to a laptop directly with Ethernet cables and synchronized with software-based precise timestamp protocol (PTP)~\cite{lixia2012software}. We run ROS drivers for Velodyne and Horizon and recorded the data in rosbag format.

\subsection{Qualitative Experiment}
 
\begin{figure}[t]
    \centering  
     \includegraphics[width=0.5\textwidth]{fig_iros/hall_traj.png}
    \caption{The trajectory result on dataset Hall. Our proposed methods show the smallest error when returning to the start point. The trajectory from different methods (bottom), the zoom-in view of starting and ending point(top left), the changes along Z-axis(top right)}
    \label{fig:hall_traj} 
\end{figure}

 \begin{table}[t]
    \centering
    \caption{End-to-end position error in meters (N/A when odometry estimations diverge; V: Velodyne VLP-16, H: Livox Horizon, I: IMU). Numbers in bold indicate the best performance, while underscored numbers indicate the second best in each environment.} 
    \begin{tabular}{@{}lccc@{}}
        \toprule 
            Dataset         & Hall   & Corridor  & Office                 \\[0.5ex]
         \midrule
            LeGo (V)    & 0.567   & 0.336   &   0.127                     \\  [0.5ex] 
            FLIO (HI/VI)      & 0.109 / \underline{0.069}  & N/A / \textbf{0.062}  & N/A / 0.188                \\  [0.5ex]  
            LIOM (HI/VI)  & N/A / 0.736     & N/A / 1.951      & NA /  \textbf{0.102}        \\  [0.5ex]  
            Ours (HI/VI)  & N/A / 0.107     & N/A / 0.132      & NA / 0.165                 \\  [0.5ex]  
            Ours (HVI)   & \textbf{0.051}  & \underline{0.085}      &  \underline{0.124}         \\  [0.5ex]   
        \bottomrule 
        \hspace{.42em}
    \end{tabular}    
    \label{table:pose_error}
\end{table} 

From our previous research~\cite{li2022dataset, sier2022benchmark}, tightly coupled solid-state lidar-inertial system show competitive performance at outdoors but poorly in indoor environments. Therefore, here we aim to compare our proposed system on typical and challenging indoor environment: office room, long corridor and large hall. The data are gathered with platform as Fig.~\ref{fig:hardware_platform} shows at ICT-City in Turku, Finland.

We compare our proposed method with several state-of-the-art SLAM algorithms: LeGO-LOAM~\cite{shan2018lego}~\footnote{https://github.com/RobustFieldAutonomyLab/LeGO-LOAM}, Fast-LIO~\cite{xu2021fast}~\footnote{https://github.com/hku-mars/FAST_LIO} and LILI-OM~\cite{li2021towards}~\footnote{https://github.com/KIT-ISAS/lili-om}. LeGO-LOAM is lidar only odometry, Fast-LIO and LILI-OM are tightly coupled lidar inertial odometry which can both work with solid state lidar and spinning lidars. Fast-LIO features with  a tightly-coupled iterated extended Kalman filter framework and iKD-tree data structure which show efficient and robust performance~\cite{xu2021fast}. Similar to our proposed method, LILI-OM employ keyframe-based sliding window optimization but only fuse signle LiDAR and  pre-integrated IMU measurements. As Fast-LIO, LI
During the experiments, we use the default configurations from official Github repository,loop closure detection are off for each methods.

We select three challenging indoor environments,  large hall, aong corridor, and office, to compare the proposed methods with selected state-of-the-art methods. To compare the odometry accuracy, all three datasets were starting and ending at same place. The mean square distance(MSE) between the starting position and ends position are treated as error. The results generated by selected methods in all dataset shows in Table~\ref{table:pose_error}. 

\subsubsection{Hall}

This data was recorded at a hall environment around 127m $\times$ 35 m to compare odometry and mapping performance in relatively large indoor environment. The recording start at a narrow space and following a 180~/degree U-turns where most of the FoV of the solid-state-lidar are covered by near walls, therefor, solid-state lidar only based methods cannot receive enough features that ight cause huge drift. 
We show our The trajectory at mapping results at Fig.~\ref{fig:hall_mapping}. From position error shown in Table~\ref{table:pose_error}, our proposed methods shows the best performance reach 5.1 centimeters, and Fast-LIO with Velodyne(V) and IMU(I) show the second best performance.

\subsubsection{Corridor}

Corridor environment is another challenging environment as low resolution lidars might cannot get enough feature points from environment to perform robust localization in environment. The data sequence recorded at a long 60 meters long corridor as mapping results shows in Fig.~\ref{fig:corridor_mapping}. The Fast-LIO(VI) shows the best and our proposed method show the second best performance.
 
\subsubsection{Office}

Another data sequence is recorded at an office room with size 12m $\times$ 3.7 m . To make the mapping task more challenging in this environment, we perform several fast 180~\degree U-turns during recording. From the result, we can see LIOM(VI) shows the best performence and our proposed methods (HVI) shows the second best.

Our proposed multi-modal lidar-inertial methods shows competitive and most robust performance between selected methods. However, as the proposed method take more measurements from the environment, in theory it should be able to outperform all others methods. Here, we try to analyse the error that may increase the error in our proposed system.  First, our time synchronization between lidars is on software level  which has sub-microsecond accuracy. The inaccurate timestamp for each point will bring the error to system during cloud un-distortion and cloud merging module that hard to eliminate.
% 2) To achieve higher resolution of maps, each frames of data are included into sliding window, this may increase the accumulating error.
% We also found Fast\_LIO(VI) also show quite robust performance. We think its because of all point cloud(not just feature cloud) are used in tightly-coupled lidar-inertial pose-estimation; and a global map are maintained with novel i-kdtree. 
The VI based method survive in all dataset sequence. However, for HI based methods failed in most of the sequence except Fast\_LIO(VI) in large hall environment. 
% 
To understand the difference of each lidars, we also test our methods with Velodyne-only odometry. The results shows the accuracy of proposed method VI is less accurate then the HVI which indicate the horizon lidar can improve the systems performence.


 \subsection{Mapping Quality Comparison}
 
 One of the key benefit of multi-lidar system is its high perception awareness ability. Here we will compare the mapping quality in terms of resolution. Part of the mapping results by our proposed methods have shown in Figure.~\ref{fig:hall_mapping} and~\ref{fig:corridor_mapping} where the color represent intensity value. From the result, we can see many objects(e.g., door, letter) and many objects.
 We compare the mapping result between our proposed method in~\ref{fig:map_details_a} and Fast\_LIO(VI) method in~\ref{fig:map_details_b} in office room environment. By zoo-in same area, we can see more uniform pointcloud from backwall and TV.
 
 
  
 
\subsection{Runtime Analysis}

Our evaluations were conducted on a laptop with an Intel Core i7-10875H CPU and 64 GB RAM on Unbuntu 18.04.6 LTS system. 
% 
Our proposed methods show real-time performance in evaluated data sets.
We show average runtime per frame in Table~\ref{tab:runtime} and feature number~\ref{tab:feature_num}.
% Preprocessing for feature extraction and scan registration was lightweight, with the runtime primarily influenced by backend fusion. 
% The process of constructing LiDAR constraints during backend fusion was found to be time-consuming. In Tab. V, we present statistics for feature extraction in LiLi-OM with typical configurations. During preprocessing, we tallied extracted features per frame, whereas we only counted associated features per keyframe during backend fusion. On average, plane features were extracted more frequently than edges due to Livox Horizon's uniform FoV coverage. 
% To ensure runtime efficiency, we down-sampled all features using a voxel grid filter before providing the LiDAR constraints.

 
     
\begin{table}[t]
    \centering
    \caption{Analysis of processing time for the different algorithm stages on an Intel i7-10875H CPU.}
    \label{tab:runtime}
    \begin{tabular}{@{}lccc@{}} 
        \toprule 
        \textbf{ }       & \textbf{Hall} & \textbf{Corridor} &  \textbf{Office} \\  
        \midrule 
        Pre-processing stage        & 4.14         & 4.44            & 4.37 \\  
        Lidar feature extraction  & 80.32        & 86.74          & 94.21 \\   
        Pose estimation, optimization     & 139.71       & 123.51         & 132.73\\  
        \bottomrule
        \hspace{.42em}
    \end{tabular}
\end{table}

\begin{table}[t]
    \centering
    \caption{Average number of feature points extracted from the different lidars in the three tested environments. Only points in a range between 1\,m and 50\,m are considered.}
    \label{tab:feature_num}
    \begin{tabular}{@{}lcccccc@{}} 
        \toprule 
        \textbf{ }       &\textbf{V-raw} & \textbf{V-edge} &\textbf{V-plane} &\textbf{H-raw} & \textbf{H-edge} &\textbf{H-plane} \\  
        \midrule 
        \textbf{Hall}    & 17947         & 257   & 15883   & 20174  & 318  & 1719\\  
        \textbf{Corridor}& 15268         & 163   & 6815    & 12698  & 228  & 3596 \\   
        \textbf{Office} & 22915          & 385   & 21032   & 23823  & 719  & 2108\\  
        \bottomrule
        \hspace{.42em}
    \end{tabular}
\end{table}

% \begin{figure*}[!htb]
% \centering
% \minipage{0.5\textwidth}
%   \includegraphics[width=\linewidth]{fig_iros/map_details_0.png}
%   \caption{A really Awesome Image}\label{fig:awesome_image1}
% \endminipage\hfill
% \minipage{0.5\textwidth}
% \centering
%   \includegraphics[width=\linewidth]{fig_iros/map_details_1.png}
%   \caption{A really Awesome Image}\label{fig_iros/map_details_1.png}
% \endminipage 
% \end{figure*}
 
% \begin{table}[h]
% \centering
% \caption{Average feature numbers}
% \label{tab:runtime}
% \begin{tabular}{|c|c|c|}
% \hline
% \textbf{ } & \textbf{Column 2} & \textbf{Column 3} \\ \hline
% pre-processing  & Row 1, Col 2 & Row 1, Col 3 \\ \hline
% scan registration  & Row 2, Col 2 & Row 2, Col 3 \\ \hline
% sliding window  & Row 3, Col 2 & Row 3, Col 3 \\ \hline
% plane extraction  & Row 3, Col 2 & Row 3, Col 3 \\ \hline 
% \end{tabular}
% \end{table}



% \begin{table*}[t]
%     \centering
%     \caption{ ATE ($\mu/\sigma$) of selected SLAM methods (N/A when odometry estimations diverge). Best results for each sequence are in bold.V:VLP-16, H:Horizon, I: built-in IMU\red{Example,TODO}} 
%     \begin{tabular}{@{}ccccccc||cc@{}}  
%     \toprule 
%         Sequence        & LEGO (V)     & LIOL (HI) & LILI_OM (HI)  & LILI_OM (VI) &Fast_LIO (HI)  &Fast_LIO (VI)  & Our (HVI)  &Our(VI)   \\[0.5ex]
%      \midrule     
%         Indoor01        & 0.497/0.328    & N/A         & N/A          & 0.315/0.220        & 1.01/0.153        & 0.132/0.022 & {\textbf0.083/0.042} & XXX \\[0.5ex] 
%         % Indoor01        & 0.497/0.328    & N/A         & N/A          & 0.315/0.220        & 1.01/0.153        & 0.132/0.022 & \textbf{0.083/0.042} &2 \\[0.5ex] 
%         % Indoor01        & 0.497/0.328    & N/A         & N/A          & 0.315/0.220        & 1.01/0.153        & 0.132/0.022 & \textbf{0.083/0.042} &2\\[0.5ex] 
%         % Indoor02        & \textbf{ 0.17 / 0.12}     &  0.34 / 0.21        & 0.70 / 0.20       &  N/A          & 0.48 /  0.17   &  N/A            \\  [0.5ex]   
%     \bottomrule 
%     \end{tabular}    
%     \label{table:ate_error}
% \end{table*} 

% \begin{table}
  
%     \centering 
%     \caption{Relative pose estimation error \red{TODO: complete data}}

%     \scalebox{0.7}{
%     \begin{tabular}{@{}c|c|cccc|cccc@{}}   
%     \toprule 
%     Seq.     & Method  & x  & y  & z &  \shortstack[c]{Total\\ Trans.(m })   & roll  & pitch  & yaw & \shortstack[c]{Total \\ Roll.(\degree)}   \\[0.5ex]
%      \midrule  
%      \multirow{6}{*}{I} %Long corridor   
%             & LeGo (V)  & -0.265    & 0.118     & 0.170     & 0.336 & -2.698    &0.271  & 1.344     &2.71 \\
%             & FLIO (HI) & -5.162    & 6.851     &  -4.201   & 9.552 &  5.400    &-1.215 & 5.319     & 5.456  \\  [0.5ex]
%             & FLIO (VI) & 0.015    &  -0.021   & -0.056    & \textbf{0.061} & 0.605     & 0.099 & -0.818    & 0.824  \\
%             % & LiOM (HI) & -         &-          & -         &-      & -         &-      &-          &- \\
%             & LiOM (VI) & -0.524    & 0.117     & -1.875    & 1.950 & 2.329     &-1.065 & -5.581    & 5.681 \\  
%             & Our (HVI) & 0.078     & 0.079     & -0.03     &0.118  & 0.057     &0.100  & 1.157     & \textbf{1.161}  \\   [0.5ex]
%      \hline
%      \multirow{6}{*}{II} % classroom   
%             & LeGo (V)   &  0.007   &  -0.031   &  -0.059   &  0.067  &  -0.233   &  -0.2   &  0.466   &  0.507 \\
%             & FLIO (HI)  &  -1.54   &  -15.396   &  -0.346  &  6.716   &  2.162   &  5.336   &  5.756 \\   
%             & FLIO (VI)&  -0.065   &  -0.056   &  -0.167   &  0.188  &  1.078   &  0.232   &  -0.512   &  0.562  \\
%             % & LiOM (HI)  & - & - & - & - & - & - & - & - \\
%             & LiOM (VI)  &  -0.041   &  0.033   &  0.087   &  0.102 &  0.483   &  0.862   &  1.137   &  1.426 \\  
%             & Our (HVI) &  0.158   &  0.022   &  -0.289   &  0.33  &  -0.114   &  -1.663   &  -1.725   &  2.395 \\  [0.5ex] 
%     \hline
%      \multirow{6}{*}{III} % Hall   
%             & LeGo (V)   &  -0.09   &  -0.535   &  0.189   &  0.574  &  5.365   &  -4.447   &  2.639   &  5.17 \\
%             & FLIO (HI)  &  -0.103   &  -0.035   &  0.023   &  0.111 &  -0.53   &  -0.871   &  -0.049   &  0.873 \\   
%             & FLIO (VI) &  \textbf{-0.013}   &  -0.036   &  \textbf{-0.015}   &  0.041  &  -0.498   &  -0.433   &  0.441   &  0.618  \\
%             % & LiOM (HI)  & - & - & - & - & - & - & - & - \\
%             & LiOM (VI)   &  0.45   &  0.371   &  -0.45   &  0.737 &  0.194   &  2.518   &  1.094   &  2.746 \\  
%             & Our (HVI)  & 0.024 & \textbf{0.022} & 0.018 & \textbf{0.037} & 0.392 & -0.304 & -1.961 & - \\   [0.5ex]
%     \bottomrule 
%     \end{tabular}    
%     } 
%     \label{table:datasets_details}
% \end{table} 

% \begin{table}[t]
%     \centering
%     \caption{ Dataset Details} 
%     \begin{tabular}{@{}ccccc@{}}  
%     \toprule 
%         Dataset     & Environment  & Scans number & Duration  & Trajectory    \\[0.5ex]
%      \midrule     
%         room01      & small office      & XXX & XXX & XXX  \\  [0.5ex] 
%         corridor01    & Long corridor   & XXX & XXX & XXX  \\  [0.5ex] 
%         corridor02    & Large Hall      & XXX & XXX & XXX  \\  [0.5ex] 
%         Hall01      & Forest Short      & XXX & XXX & XXX  \\  [0.5ex]
%         % Forest02    & Forest Long       & XXX & XXX & XXX  \\ 
%     \bottomrule 
%     \end{tabular}    
%     \label{table:data_details}
% \end{table} 
 
